A PTAS for a Class of Stochastic Dynamic Programs

We develop a framework for obtaining polynomial time approximation schemes (PTAS) for a class of stochastic dynamic programs. Using our framework, we obtain the first PTAS for the following stochastic combinatorial optimization problems: \probemax: We are given a set of $n$ items, each item $i\in [n]$ has a value $X_i$ which is an independent random variable with a known (discrete) distribution $\pi_i$. We can {\em probe} a subset $P\subseteq [n]$ of items sequentially. Each time after {probing} an item $i$, we observe its value realization, which follows the distribution $\pi_i$. We can {\em adaptively} probe at most $m$ items and each item can be probed at most once. The reward is the maximum among the $m$ realized values. Our goal is to design an adaptive probing policy such that the expected value of the reward is maximized. To the best of our knowledge, the best known approximation ratio is $1-1/e$, due to Asadpour \etal~\cite{asadpour2015maximizing}. We also obtain PTAS for some generalizations and variants of the problem and some other problems.

==> a_probek.tex <==

\section{Committed \probek~Problem}
In this section, we prove Theorem \ref{thm:topk_commit}, \ie obtaining a PTAS for the committed \probek~problem. On the committed model, we are committed to making an irrevocable decision immediately whether to pick it or not whenever we probe an item. If we add the item to the output set $C$, the profit is collected. Otherwise, no profit is collected and we are going to probe the next item.
%Similarly, the process of applying a policy $\sigma$ on an instant $\pi$ can be represented as a binary decision tree $T(\sigma,\pi)$. Each node $v$ in $\cT_{\sigma}$ is labeled by a unique random variable $X_{v}$. It has two children---
%\subsection{$\probemax$ on Committed Model}
\begin{thm}
There is a polynomial time algorithm that finds a committed policy with the expected value at least $(1-\ep)\opt$ for the committed \probek~problem. 
\end{thm}



\begin{proof}
Let $\sigma^{\ast}$ be the optimal committed policy. Suppose $\sigma^{\ast}$ is going to probe the next item $i$ and choose $i$ if $X_i$ realizes to a value $\theta\in S$. Then $\sigma^{\ast}$ would choose  $i$ if $X_i$ realizes to a larger value $s\ge \theta$. We call $\theta$ threshold for the item $i$. 
Thus the committed policy $\sigma^{\ast}$ for the committed \probek~problem can be represented a decision tree $\cT(\sigma^{\ast},\pi)$.  Every node $v$ is labeled by an unique item $i(v)$ and  a threshold $\theta(v)$, which means the policy accepts the item $i(v)$ and if $X_v$ realizes to a size $s\ge \theta(v)$, and otherwise rejects it. It can be equivalently viewed as a Bernoulli case where  each item $i$ has weight $w_i=\bE[X_i\,|\,X_i\ge \theta]$ and is ``active'' with probability $p_i=\Pr[X_i\ge \theta]$.

Now, we present a stochastic dynamic program for this prolem. For each item $i$, we create a set of actions $\cB_i=\{b_{i}^{\theta}\}$, where $b_{i}^{\theta}$ represents the action that we probe the item $i$ with the threshold $\theta$. Since we  assume discrete distribution, there are at most a polynomial number thresholds. Hence the set of action $\cA=\cup_{i\in[n]}\cB_i$ is bounded by a polynomial. The only requirement is that at most one action from $\cB_i$ can be selected, which implies that all feasible sets of actions we can take form a partition matroid (see Section \ref{sec:partition}). We set $\cS=\{0,1,\ldots,k\}$, $T=m$ and $I_1=0$. When we select an action $b_i^{\theta}$ and observe its value realization, say $X_i$, we define the system dynamic functions to be
\begin{equation}
I_{t+1}=f(I_t,b_i^{\theta})=
\left\{
\begin{array}{cl}
I_k+1   & \text{if } X_i\ge \theta \text{ and } I_k<k,\\
I_k & \text{otherwise; } 
\end{array}
\right.
,\quad
g(I_t,b_i^{\theta})=
\left\{
\begin{array}{cl}
X_i   & \text{if } X_i\ge \theta \text{ and } I_k<k,\\
0 & \text{otherwise;}
\end{array}
\right.
\end{equation}
for $I_t\in \cS$ and $t=1,2,\ldots,n$, and $h(I_{T+1})=0$.  Then Assumption \ref{cond:main} is immediately satisfied. By Theorem \ref{thm:main}, we can find a policy $\sigma$ with profit at least
$$
\opt-O(\ep)\cdot\mopt=\left(1-O(\ep)\right)\opt,
$$   
where $\opt$ denotes the expected profit of the optimal policy for the committed \probek~problem and $\mopt=\mmopt=\DP^{\ast}(0)=\opt$. 
\end{proof}

\section{Committed \pandora Problem}
In this section, we prove Theorem \ref{thm:pandora_commit}, \ie obtaining a PTAS for the committed \pandora problem. 
%On the committed model, we are committed to making an irrevocable decision immediately whether to pick it or not whenever we probe an item. If we add the item to the output set $C$, the profit is collected. Otherwise, no profit is collected and we are going to probe the next item.
%Similarly, the process of applying a policy $\sigma$ on an instant $\pi$ can be represented as a binary decision tree $T(\sigma,\pi)$. Each node $v$ in $\cT_{\sigma}$ is labeled by a unique random variable $X_{v}$. It has two children---
%\subsection{$\probemax$ on Committed Model}
\begin{thm}
There is a polynomial time algorithm that finds a committed policy with the expected value at least $(1-\ep)\opt$ for the committed \pandora problem. 
\end{thm}
\begin{proof}
This can be proved by an analogous argument as Theorem \ref{thm:topk_commit}.
Again, for each item $i$, we create a set of actions $\cB_i=\{b_{i}^{\theta}\}$, where $b_{i}^{\theta}$ represents the action that we probe item $i$ with threshold $\theta$. 
%The only requirement is that at most one action from $\cB_i$ can be selected. Since we  assume discrete distribution, there are at most a polynomial number thresholds. Hence the set of action $\cA=\cup_{i\in[n]}\cB_i$ is bounded by a polynomial.
 We set $\cA=\cup_{i\in[n]}\cB_i$, $\cS=\{0,1,\ldots,k\}$, $T=n$ and $I_1=0$. When we select an action $b_i^{\theta}$ and observe its value realization, say $X_i$, we define the system dynamic functions to be
\begin{equation}
I_{t+1}=f(I_t,b_i^{\theta})=
\left\{
\begin{array}{cl}
I_k+1   & \text{if } X_i\ge \theta \text{ and } I_k<k,\\
I_k & \text{otherwise; } 
\end{array}
\right.
,\quad
g(I_t,b_i^{\theta})=
\left\{
\begin{array}{cl}
X_i-c_i   & \text{if } X_i\ge \theta \text{ and } I_k<k,\\
-c_i & \text{otherwise;}
\end{array}
\right.
\end{equation}
for $I_t\in \cS$ and $t=1,2,\cdots,n$, and $h(I_{T+1})=0$. Notice that we never take an action $b_i^{\theta}$ at state $I_t$ if $\bE[g(I_t,b_i^{\theta})]<0$. Then Assumption \ref{cond:main} is immediately satisfied. By Theorem \ref{thm:main}, we can find a policy $\sigma$ with profit at least
$$
\opt-O(\ep)\cdot\mopt=\left(1-O(\ep)\right)\opt,
$$   
where $\opt$ denotes the expected profit of the optimal policy for the committed \pandora~problem and $\mopt=\mmopt=\DP^{\ast}(0)=\opt$. 

\end{proof}

